Prompt Tuning GPT-2 language model for parameter-efficient domain adaptation of ASR systems

Automatic Speech Recognition (ASR) systems have found their use in numerous industrial applications in very diverse domains creating a need to adapt to new domains with small memory and deployment overhead. In this work, we introduce domain-prompts, a methodology that involves training a small number of domain embedding parameters to prime a Transformer-based Language Model (LM) to a particular domain. Using this domain-adapted LM for rescoring ASR hypotheses can achieve 7-13% WER reduction for a new domain with just 1000 unlabeled textual domain-specific sentences. This improvement is comparable or even better than fully fine-tuned models even though just 0.02% of the parameters of the base LM are updated. Additionally, our method is deployment-friendly as the learnt domain embeddings are prefixed to the input to the model rather than changing the base model architecture. Therefore, our method is an ideal choice for on-the-fly adaptation of LMs used in ASR systems to progressively scale it to new domains.

==> ablation.tex <==
\section{Ablations}
\label{sec:abl}

% This helps us conclude the significance of learning \dop{} for domain adaptation in ASR systems. It not only helps to reduce the memory and training time costs but also performs better than fine-tuning for low-resource domains. 


% We further ran experiments to compare model performance on different 
% The above experiment proves us the effectiveness of prompt-tuning in domain adaptation. With comparable perplexity as fine-tuning, it is natural to expect that prompt-tuned model can perform at par with fully tuned model in domain specific rescoring of n-best hypothesis from an AM model in any ASR system. We verify this empirically by using the above models as first pass rescorers on an internal fastfood audio dataset for a hybrid AM model and measuring the Content Word Error Rates (CWER). While the fine-tuned version brings a relative improvement of 7.3\% over the no-adaptation baseline, training just 10 prompt tokens could already achieve 5.8\% relative improvement. Also, with 400 prompt tokens, we could almost exactly match the CWER of fine-tuned model. Since, ASR systems are used in tens of different domains, one can achieve a significant reduction in LMs that one need to maintain, by keeping a single copy of the base version of the model and saving the domain-specific prompt token embeddings. 




==> experiments-old.tex <==


In each of our experiments, we essentially compare three different approaches. The first one is our baseline of using out-of-the-box pretrained LM (called no-adaptation). This represents the performance of the model with no additional overhead in compute and memory costs for each domain. The next is our proposed approach of using \dop which have some reasonable number of additional parameters for each domain. The third one is adapting all the parameters of the pretrained LM (called fine-tuning). This approach is expected to perform the best but is not practically feasible for a ASR system serving multiple domains. 

% perplexity experiments
We design first set of experiments as a proof of concept to show that our method is capable of doing domain adaptation of the LM. For this, we used textual data from different domains of the publically available MultiDoGo dataset \cite{peskov-etal-2019-multi}. We split the data from each domain into train, dev and test. Then for each domain individually, we fine-tune (and prompt-tune) a pretrained GPT-2 \cite{radford2019language} using the train set, tune the hyper-parameters using dev set and compute the perplexity numbers on the test set. We then compare the three methods described above for different performance, memory and training time metrics. Rather than fixing the size of the \textit{domain-prompt}, we repeat the above experiment with different sizes to show how we can control the trade-offs between performance and costs using this hyper-parameter. Although, we summarize the results for one such domain (fastfood) in Fig. \ref{fig:comp}, the results are consistent across different domains. All the experiments were conducted using a machine with 16 Tesla K80 GPUs and the reported times are wall clock times in seconds. As we can see in Fig. \ref{fig:comp}, with as little as 5 prompt-tokens, the perplexity improves from 130 in out-of-the-box model (green line) to 37. With 400 prompt-tokens, we achieve a very similar perplexity to fully fine-tuned model (red line) but using orders of magnitude smaller number of learnable parameters. As one might expect, with increase in size of prompts, the performance improves but so do the memory and computation costs. We also provide text generated from the three approaches for airlines domain in Table ~\ref{table:gentext} to validate that \dop is able to generate coherent sentences related to domain similar to fine-tuned model. 

\begin{table}[]
\footnotesize
\begin{tabular}{|l|l|}
\hline
Input prompt                   & "hello how are you"                                                                                                                                                              \\ \hline
no-adaptation    & \begin{tabular}[c]{@{}l@{}}hello how are you doing?\\ I'm really happy with the results.  \end{tabular}             \\ \hline
fine-tuned  & \begin{tabular}[c]{@{}l@{}}hello how are you able to get a new flight \\ I'm flying from London Heathrow to Dubai \end{tabular} \\ \hline
domain-prompts & \begin{tabular}[c]{@{}l@{}}hello how are you able to get a refund on the flight\\ I'm flying from Glasgow to Madrid today\end{tabular}                    \\ \hline
\end{tabular}
\label{table:gentext}
\caption{Generated text for airlines domain}
\end{table}


% WERR improvements
After validating our hypothesis regarding effectively priming the model, we run experiments to solve the problem at hand of scaling the use of transformer-based neural language models to domain-specific ASR systems. For this, we use our internal dataset consisting of conversational audio utterances and transcriptions from multiple domains like airlines, insurance etc for evaluation of different approaches which is representative of the common ASR application in task-oriented dialog systems. We use another internal dataset which consists of conversational text utterances from each of the above domains that can be used for learning the \dop or doing fine-tuning. 
% Wherever specified, we also use open-source dialogue dataset DSTC8 \cite{} for pretraining  to bias out-of-the-box GPT-2 to conversational data. 
On our evaluation data, we compute the nbest hypothesis from an ASR system and then run rescoring using different versions of GPT-2 model as an external LM. We compare domain-adaptation approaches on metrics like Content Word Error Rate (CWER). CWER is a more relevant metric for domain-specific ASR systems as it disregards common English words for WER computation and hence represents performance on domain-specific vocabulary. All the numbers reported in this paper are CWER Relative \% (CWERR) which represents improvement in performance over the baseline of rescoring with out-of-the-box GPT-2 
% (no-adaptation).  

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/ablation.png}
    \caption{Comparing the performance of different domain prompt sizes and fine-tuning}
    \label{fig:size}
\end{figure*}

Rather than fixing the \dop size or the amount of domain-specific training data available or the domain, we evaluate our methodology across all possible combinations to fully understand the trade-offs. 
Fig. \ref{fig:size} summarizes the results for 3 domains ie finance, insurance and travel. The x-axis represents the number of in-domain training sentences used for adapting. The y-axis is the CWERR \% relative to the no-adaptation baseline. Different lines represent different sizes of \dop as well there is a dashed-line for fine-tuning. There are multiple important observations to make from the plots. 
First, the obvious ones that the performance generally improves for all the models with increase in the training data across all domains and that performance generally improves with increase in size of the \dop. 
Next, we observe that using \dop not only helps to save memory and training time costs, but also improve performance over fully-fine-tuned models in low data settings. When the number of domain-specific dataset is in the orders of few hundreds to thousands, \dop are able to better adapt the pretrained model than fine-tuning each of millions of parameters. This setting represents very common practical application where limited amount of conversational domain-specific data is available for ASR in dialog systems. \dop with size as small as 5 with handful of trainable parameters are representative enough to learn domain-specific details, whereas fine-tuned model overfits to the few examples provided and perform worse than the out-of-the-box GPT2 model.  However, as expected, as the size of training data increases to very large amount, fine-tuning models start to perform better than \dop models. This comes at the cost of memory, training time and data-collection. The results showcased in this plot can potentially help any domain-specific ASR system developer to efficiently trade-off costs and performance based on the amount of training data available for the domain in hand. Particularly, for a new domain with limited data, using a simple 20-token domain-prompt prefix can give 3-6\% CWEER improvement over the baseline of common pre-trained GPT-2 model, where naive fine-tuning is not even a choice (because of overfitting). 


As mentioned in the Sec.~\ref{sec:meth}, we initialized the \dop with most common vocabulary words. In table ~\ref{table:comp}, we run an ablation on how much does this choice of initialization contribute to the performance. The following analysis was done using \dop of size 50, one initialized randomly and the other using common vocabulary words. We see that using the latter, consistently helps to improve performance across different domains. We attribute this to the hypothesis that beginning with embeddings closer to domain-specific words helps self-attention in these LM architectures to better encode sentences.





\begin{table}[]
\footnotesize
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Domain}     & \multicolumn{2}{c|}{\textbf{CWERR  \%}}    \\ \hline
\textbf{}           & \textbf{Random Init} & \textbf{Vocab Init} \\ \hline
\textbf{finance}    & -0.4                 & 4.14                \\ \hline
\textbf{travel}     & 2.2                  & 3.97                \\ \hline
\textbf{insurance}  & 1.08                 & 2.03                \\ \hline
\textbf{airlines}   & 4.81                 & 9.91                \\ \hline
\textbf{mediacable} & 0.57                 & 0.83                \\ \hline
\end{tabular}
\label{table:comp}
\caption{Choice of initialization for \dop}
\end{table}



% \begin{table}[]
% \footnotesize
% \begin{tabular}{lrr}
% \hline
%           & \multicolumn{1}{l}{{Vocabulary Initialization}} & \multicolumn{1}{r}{{Random Initialization}} \\ \hline
%           & \multicolumn{2}{c}{CWER Relative \% to no-adaptation baseline}                                                   \\
% airlines   & \textbf{15.36 }                                                & --                                                   \\
% finance    & 0.98                                                  & \textbf{--     }                                                \\
% insurance  & 0.31                                                  & \textbf{--      }                                              \\
% mediacable & \textbf{3.18 }                                                 & --                                                   \\
% retail     & -9.58                                                 & \textbf{--}                                                   \\
% healthcare & -5.75                                                 & \textbf{--  }                                                   \\ \hline
% \end{tabular}
% \label{table:comp}
% \caption{Choice of initialization for \dop}
% \end{table}

% However, the improvement is bigger for models with larger number of trainable parameters. Therefore, with the increase in the size of the training data, these methods start to perform better such that eventually fine-tuning (with orders of magnitude more parameters) performs better than \dop with very large amount of domain data. Analogously, in the limited data regime, models with smaller prompt-sizes adapt faster while fine-tuning performs worse than the baseline due to over-fitting. This experiment clearly lays out that using \dop not only helps to reduce the memory and training time costs but also performs better than other alternatives in low-resource domains. 

% Next, we run different ablation studies to better understand the difference in performance between fine-tuning and \dop methods. No doubt, the purpose of introducing \dop is not to always beat the fine-tuning method but to achieve comparable performance with limited number of parameters. Our first set of ablations is focused on different prompt-sizes and different amount of training data for a domain. This experiment has practical significance as generally different \section{Experiments}
\label{sec:exp}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/perp.png}
    \caption{Comparing the performance, computation and memory costs of different methods of domain adaptation}
    \label{fig:comp}
\end{figure*}amount of textual data is available for different domains and size of the \dop provides a control to balance the performance and costs trade-off to the system developer. 

















% In table \ref{table:comp}, we summarize the comparison between fine-tuning and \dop for different domains. For this experiment, we use 4000 training examples from each of the domain for both the domain-adaptation approaches. This setting represents very common practical application where limited amount of conversational domain-specific data is available for ASR in dialog systems. As we can see, the fine-tuned models overfit to the limited data because there are large number of parameters to adapt. On the other hand, we use \dop of size 50, as it has significantly less number of trainable parameters but are representative enough to learn domain-specific details. Therefore, we see an improvement over the baseline for almost all the domains, and sometimes, a better CWER than even fully-fine-tuned models. As mentioned in Sec. \ref{sec:meth}, we initialize the prompt embedding with the most common vocabulary words from the domain. With very little overhead in both memory and training time, we achieve a CWERR of around 11\% over the baseline in airlines domain. 


% \begin{table}[]
% \begin{tabular}{lrr}
% \hline
%           & \multicolumn{1}{l}{{ Finetuning}} & \multicolumn{1}{r}{{ Prompt-tuning}} \\ \hline
%           & \multicolumn{2}{c}{CWER Relative \% to no-adaptation baseline}                                                   \\
% airlines   & \textbf{15.36 }                                                & 10.90                                                    \\
% finance    & 0.98                                                  & \textbf{3.71     }                                                \\
% insurance  & 0.31                                                  & \textbf{1.45       }                                              \\
% mediacable & \textbf{3.18 }                                                 & -0.37                                                    \\
% retail     & -9.58                                                 & \textbf{0.73  }                                                   \\
% healthcare & -5.75                                                 & \textbf{0.00  }                                                   \\ \hline
% \end{tabular}
% \label{table:comp}
% \caption{\dop vs fine-tuning}
% \end{table}



